On Mixing Distributions Via Random Orthogonal Matrices and the Spectrum of the Singular Values of Multi-Z Shaped Graph Matrices

In this paper, we introduce and analyze a new operation $\circ_{R}$ which mixes two distributions $\Omega$ and $\Omega'$ via a random orthogonal matrix. In particular, we take $\Omega \circ_R \Omega'$ to be the limit as $n \to \infty$ of the distribution of singular values of $DRD'$ where $D$ and $D'$ are $n \times n$ diagonal matrices whose diagonal entries have distributions $\Omega$ and $\Omega'$ respectively and $R$ is a random $n \times n$ orthogonal matrix. We show that $\circ_R$ has several nice properties. We first observe that $\circ_R$ is commutative and associative and compute the moments of $\Omega \circ_R \Omega'$ in terms of the moments of $\Omega$ and $\Omega'$. We then show that $\circ_R$ interacts very nicely with the spectrum of the singular values of Z-shaped and multi-Z-shaped graph matrices. This allows us to answer the question posed by our previous paper of how to describe the spectrum of the singular values of Z-shaped and multi-Z-shaped graph matrices when the input distribution is not $\{-1,1\}$. In our analysis, we show that the moments of our distributions are closely connected to non-crossing partitions and prove a number of new results on non-crossing partitions which may be of independent interest.

==> delete.tex <==
%%%%%%%%%%%%%%%%% Introduction %%%%%%%%%%%%%%%%%%%%%
\begin{defn}
    We define $\mathbf{\o}$ to be the set of all random distributions and $\oset$ to be the set of distributions $\o$ with mean $0$ and variance $1$. 
\end{defn}

\begin{cor}\label{cor:main-1}
    $\image\(\opr\)\subseteq \oset$. i.e. $\opr$ can be viewed as $\oset\times\oset \to \oset$.
\end{cor}
\begin{proof}
    $\o\opr\o'$ has mean $0$ since
    \begin{align*}
        \(\o\opr\o'\)_{1} 
        =& \Ebb\[\trace\(DRD'\)\] 
        = \Ebb\[ \sum_{i,j_1,j_2\in [n]} d_{i,j_1} R_{j_1,j_2} d'_{j_2,i}\] 
        = \sum_{i,j_1,j_2\in [n]} \Ebb\[ d_{i,j_1} R_{j_1,j_2} d'_{j_2,i}\] \\
        =& \sum_{i,j_1,j_2\in [n]} \Ebb\[ d_{i,j_1}\] \Ebb\[ R_{j_1,j_2}\] \Ebb\[ d'_{j_2,i}\] = 0\,.
    \end{align*}
    The last step is because $\o\in \oset$ and thus $\Ebb\[d_{i,j_1}\]=0$ for any $i,j_1$.
    
    By \Cref{thm:main-1-circ}, $\displaystyle \(\o\opr\o'\)_{2} = C\(\o_2,\o_2'\)\cdot \o_2\o_2' = (-1)^2\cdot 1\cdot {1+1-2\choose 0} = 1$. Thus $\variance\(\o\opr\o'\) = \(\o\opr\o'\)_{2} - \(\(\o\opr\o'\)_{1}\)^2 = 1-0 = 1$.
\end{proof}

Given a shape $\a$ associated with distributions $\oa$, a graph $G=\(V(G),E(G)\)$ and an injective map $\sigma: V(\alpha) \to V(G)$, we define $\chi_{\sigma(E(\a))}(G) = \prod_{e \in E(\a)} x_{\sigma(e)}^{e}$ where each \textit{edge variable} $x_{\sigma(e)}^e$ is sampled independently from $\o_e$.

We can prove \Cref{thm:main-0} using the Trace Power Method:
\main*

\begin{proof}
    By the Trace Power Method, it suffices to match the trace power moments of two matrices to prove their limiting distributions of the singular values are the same. Thus
    \begin{enumerate}
        \item $\o\circ_R\o' = \o'\circ_R \o$: since $\(DRD'\)^T = D'R^TD$ and $\trace\(\(MM^T\)^k\) = \trace\(\(M^TM\)^k\)$, therefore 
        \begin{equation*}
            \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(M_1M_1^T\)^k\)\] = \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(M_2{M_2}^T\)^k\)\]
        \end{equation*}
        where $M_1=DR_1D'$, $M_2=D'R_2D$ and $D$ and $D'$ are $\o$ and $\o'$-distribution diagonal matrices, respectively.
        
        \item $\(\o\circ_R \o'\)\circ_R \o'' = \o\circ_R \(\o'\circ_R\o''\)$: we will prove that $DR_1\(D'R_2D''\)$ has the same trace power moments as $DR_3\hat{D}$ where $\hat{D}$ is the $\o'\circ_R\o''$-distribution diagonal matrix. Let $M = D'R_2D''$. Since $\o'\circ_R\o''$ is the singular value spectrum of $M$, $M = U\hat{D}V^T$ for some orthogonal matrices $U$ and $V$. We have $MM^T = \(U\hat{D}V^T\) \(V\hat{D}U^T\) = U\hat{D}^2U^T$, thus
        \begin{align*}
            & \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\(DR_1M\)\(DR_1M\)^T\)^k\)\] \\
            =& \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(DR_1\(MM^T\)R_1^TD\)^k\)\] \\
            =& \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(DR_1 U\hat{D}^2U^TR_1^TD\)^k\)\]\\
            =& \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\(D\(R_1U\)\hat{D}\)\(D\(R_1U\)\hat{D}\)^T\)^k\)\]\\
            =& \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\(DR_3\hat{D}\)\(DR_3\hat{D}\)^T\)^k\)\] 
            \text{ since } R_1U \text{ is a random orthogonal matrix}
        \end{align*}
        
        Similarly, we can prove that $\(DR_1D'\)R_2D''$ has the same trace power moments as $\bar{D}R_3D''$ where $\bar{D}$ is the $\o\circ_R\o'$-distribution diagonal matrix. 
        
        Since $\(DR_1D'\)R_2D'' = DR_1\(D'R_2D''\)$, $\bar{D}R_3D''$ and $DR_3\hat{D}$ have the same trace power moments and thus same limiting distribution of singular values, so by definition $\(\o\circ_R \o'\)\circ_R \o'' = \o\circ_R \(\o'\circ_R\o''\)$ as wanted.
    \end{enumerate}
\end{proof}

%%%%%%%%%%%%%%%% Preliminaries %%%%%%%%%%%%%%%%%%
\begin{defn}\label{defn:*-algebra}
    We say that a unital algebra $\A$ over $\Cbb$ is a \emph{$*$-algebra} if $\A$ is associated with a $*:\A\to\A$ operation where 
    \begin{enumerate}
        \item $(a+b)^* = a^* + b^*$ for any $a,b\in\A$
        \item $(ab)^* = b^*a^*$ for any $a,b\in\A$
        \item $(a^*)^* = a$ for any $a\in\A$
        \item ${1_{\A}}^* = 1_{\A}$
        \item $*$ is \emph{antilinear}: $(c a)^* = \bar{c} a^*$ for any scalar $c\in\Cbb$ and $a\in\A$,. 
    \end{enumerate}
\end{defn}

\begin{defn}\label{defn:*-prob-space}
    We say that $\(\A,\varphi\)$ is \emph{$*$-probability space} if $\(\A,\varphi\)$ is a non-commutative probability space, $\A$ is a $*$-algebra, and $\varphi(a^*a) \geq 0$ for any $a\in\A$. We say that $\varphi$ is \emph{positive} if the last condition holds.
\end{defn}

\begin{defn}\label{defn:C*-algebra}
    We say a unital algebra $\A$ over $\Cbb$ is a \emph{$C^*$-algebra} if $\A$ is a $*$-algebra and $\A$ is associated with a norm $\norm{\cdot}:\A\to \Rbb_{\geq 0}$ such that $\(\A, \norm{\cdot}\)$ is a complete normed space and 
    \begin{enumerate}
        \item $\norm{a\cdot b}\leq \norm{a}\cdot \norm{b}$ for any $a,b\in \A$
        \item $\norm{a^*a} = \norm{a}^2$ for any $a\in \A$.
    \end{enumerate}
\end{defn}

\begin{defn}\label{defn:C*-prob-space}
    We say that $\(\A,\varphi\)$ is a \emph{$C^*$-probability space} if $\(\A,\varphi\)$ is a $*$-probability space and $\A$ is a $C^*$-algebra.
\end{defn}

\begin{eg}
    $\(M_n\(\Cbb\), \trace\)$ is a $C^*$-probability space where $\trace$ is the normalized trace $\trace(A) = \frac{1}{n}\(a_{11}+\dots + a_{nn}\)$, $A^* = \bar{A}^{\,T}$ and $\displaystyle \norm{A} = \max_{\norm{v}_2 = 1} {\norm{Av}}_2$.
\end{eg}

\begin{defn}[Partition]\label{defn:partition}
    A \emph{partition} of $[n]$ is $\P=\lcurb P_1,\dots, P_m \rcurb$ where $\displaystyle\bigsqcup_{i=1}^m \; P_i = [n]$ for each $i\in[m]$.
    
    We say a partition $\P=\lcurb P_1,\dots, P_m \rcurb$ is \emph{of parts with sizes $(n_1,\dots,n_m)$} if $\abs{P_i}=n_i$ for all $i\in[m]$.
    
    We say a partition $\P=\lcurb P_1,\dots, P_m \rcurb$ is \emph{non-crossing} if there do not exist $a<b<c<d$ such that $a,c\in P_i$ and $b,d\in P_j$ for some $i\neq j\in[m]$.
    
    We denote the set of all partitions of $[n]$ as $\P_n$, and the set of non-crossing ones as $\np_n$.
\end{defn}

\begin{rmk}
    Given a non-crossing partition $\P$ of $[n]$, we can visualize the partition $\P=\{P_1,\dots,P_m\}$ as placing polygons of size $\abs{P_i}$ non-crossingly on a cycle of length $n$. When $\abs{P_i}=1$, the corresponding polygon is simply a point.
\end{rmk}

\begin{rmk}
    Given $\vaa\in P_k$ and $\P\in\np\(\vaa\)$, we can visualize $\P$ as placing $\a_i$ polygons of size $i$ on the cycle $\C_k$ non-crossingly.
\end{rmk}

\begin{eg}
    Consider the partition $\P=\left\{\{2\},\{4\},\{6\}, \{1,3\}, \{5,7,8\}\right\}$ of $[8]$. Then $\P$ can be represented as placing the line $\{4,6\}$ and the triangle $\{5,7,8\}$ on the cycle $\C_8$ as shown in \Cref{fig:noncrossing-polygons}.
    
    \begin{figure}[hbt!]
        \centering
        \includegraphics[scale=0.35]{images/noncrossing-polygons.png}
        \caption{$\{1,3\}$ represents a line, and $\{5,7,8\}$ represents a triangle and all others are points.}
        \label{fig:noncrossing-polygons}
    \end{figure}
\end{eg}

\begin{defn}\label{defn:partition-alpha}
    Given $\vaa = \(\a_1,\dots,\a_k\)\in P_k$, let
    \begin{enumerate}
        \item $\P\(\vaa\)$ denotes the set of all partitions of $[k]$ into parts of sizes $\(\underbrace{1,\dots,1}_{\a_1\text{ times}}, \underbrace{2,\dots,2}_{\a_2 \text{ times }},\dots, \underbrace{k,\dots,k}_{\a_k \text{ times}}\)$,
        \item $\np\(\vaa\)\subseteq \P\(\vaa\)$ denotes the set of non-crossing partitions.
    \end{enumerate}
\end{defn}

%%%%%%%%% Prem: Restatement %%%%%%%%%%%
Using the Trace Power Method, $\displaystyle \(\o\circ_R\o'\)_{2k} =  \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(MM^T\)^k\)\]$ where $M=DRD'$.

Furthermore, under the free probability theory, we can re-express our theorem as the following. Consider $A_n = {D_n}^2$, $B_n = R_n{D_n'}^2R_n^T$. If we let $\varphi = \trace\otimes \Ebb$ (note here $\trace$ is the normalized trace), then 
    \begin{align*}
        \lim_{n\to\infty} \dfrac{\,1\,}{n}\cdot \Ebb\[\trace\(\(MM^T\)^k\)\] 
        =& \lim_{n\to\infty} \Ebb\[\dfrac{\,1\,}{n}\trace\(DR{D'}^2R^T D^2 R{D'}^2R^T \dots D^2 R{D'}^2R^T D\)\] \\
        =& \lim_{n\to\infty} \Ebb\[\dfrac{\,1\,}{n}\trace\(D^2 \(R{D'}^2R^T\) D^2 \(R{D'}^2R^T\) \dots D^2\(R{D'}^2R^T\)\)\]\\
        =& \lim_{n\to\infty} \Ebb\[\dfrac{\,1\,}{n}\trace\( A_nB_n A_nB_n\dots A_n B_n\)\]\\
        =& \lim_{n\to\infty} \trace\otimes\Ebb \(A_nB_n\dots, A_nB_n\) = \lim_{n\to\infty} \varphi\(A_nB_n\dots, A_nB_n\)
    \end{align*}
    
Thus, \Cref{thm:main-1-circ} can be reformulated in the following way.

%By \Cref{thm:free-independence-matrices}, $A_n$ and $B_n$ are asymptotically free as $n\to \infty$. Thus by \Cref{thm:cumulants}, 
%\begin{align*}
%    \lim_{n\to\infty} \varphi\(A_nB_n\dots, A_nB_n\) =  \sum_{\pi\in NC(n)} \kappa_{\pi}[A_n,\dots, A_n]\cdot \varphi_{K(\pi)} [B_1,\dots, B_n]
%\end{align*}

\begin{restatable}{thm}{mainone}
\label{thm:main-1}
Let $R_n$ be $n\times n$ random orthogonal matrix, $D_n$ and $D_n'$ be $n\times n$ random diagonal matrices where the diagonal elements are drawn independently from distributions $\Omega$ and $\Omega'$, respectively. Let $A_n = {D_n}^2$, $B_n = R_n{D_n'}^2R_n^T$, and $\varphi = \trace\otimes \Ebb$. Then
\begin{equation}
    \(\o\opr \o'\)_{2k} = \lim_{n\to\infty} \varphi\(A_nB_n\dots A_nB_n\) = \sum_{\vaa, \vbb\in P_k} C\(\vaa,\vbb\)\cdot \vec{\o}^{\vaa}\cdot \vec{\o'}^{\vbb}
\end{equation}
where if we let $a= \a_1+\dots +\a_k$ and $b=\b_1+\dots +\b_k$,
\begin{equation}
    C\(\vaa,\vbb\) = (-1)^{k+a+b-1}\cdot k\cdot \binom{a+b-2}{k-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \dfrac{(b-1)!}{\b_1!\dots\b_k!}\;.
\end{equation}
\end{restatable}


\begin{restatable}{thm}{mainone}
\label{thm:main-1}
Let $M=DRD'$ where $R$ is an $n\times n$ random orthogonal matrix, $D$ and $D'$ are $n\times n$ random diagonal matrices where the diagonal elements are drawn independently from distributions $\Omega$ and $\Omega'$, respectively. Denote $\vec{\a}=(a_1,\dots,\a_k)$ and $\vec{\b}=(\b_1,\dots,\b_k)$. Then
    \begin{align*}
        \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(MM^T\)^k\)\]
        = \sum_{\vec{\a}, \vec{\b}\in P_k} C\(\vaa,\vbb\)\cdot \voo^{\,\vaa}\cdot \vv{\o'}^{\,\vbb}
    \end{align*}
    where if we let $\a_1+\dots+\a_k=a$ and $\b_1+\dots+\b_k=b$, then
    \begin{equation}
        C\(\vaa,\vbb\) = (-1)^{k+a+b-1}\cdot k\cdot \binom{a+b-2}{k-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \dfrac{(b-1)!}{\b_1!\dots\b_k!}\;.
    \end{equation}
    
    In particular, note that $C\(\vaa,\vbb\)=0$ if $a+b\leq k$.
\end{restatable}

\begin{defn}\label{defn:mzshape-sdistr-grid-matrix}
    Given $\o^{(1)},\dots,\o^{(s)}$, consider the random matrix $\mzshapesdistr$ obtained inductively on $s$ as the following:
\begin{enumerate}
    \item $M_{Z(m),0} = D$ where $\o=\ozm$.
    \item $M_{Z(m),1} = D'RD$ where $\o'= $ the limiting distribution of singular values of $M_{Z(m),0}$ and $\o=\o^{(1)}$. %i.e. $\o_{2i}' = C(i,m)$ for all $i$.
    \item $M_{Z(m),i} = D'RD$ where $\o'=\o_{Z(m),\o^{(1)},\dots,\o^{(i-1)}}:=$ the limiting distribution of singular values of $M_{Z(m),i-1}$ and $\o=\o^{(i)}$ for $i=1,\dots,s$.
\end{enumerate}
\end{defn}

\begin{equation}
    \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\mzshapesdistr{\mzshapesdistr}^T\)^{k}\)\] = \lim_{n\to\infty}\, \dfrac{\,1\,}{r(n,m)}\cdot\Ebb\[\trace\(\(M^{(G)}_{Z(m),s}{M^{(G)}_{Z(m),s}}^T\)^{k}\)\] 
\end{equation}
for all $k\geq 0$.

Consider the random matrix $\mmzshape = D'RD$ where $\o'=\ozmm$ and $\o=\ozm$. Let $\displaystyle r(n,m)=\dfrac{n!}{(n-m)!}$ Then for each $k\in \Nbb$,
\begin{equation}
\begin{aligned}
    \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb&\[\trace\(\({\mmzshape}^T\mmzshape\)^{k}\)\] = C\(k,m+m'\) \\
    =& \lim_{n\to\infty}\, \dfrac{\,1\,}{r\(n,m+m'\)}\cdot\Ebb\[\trace\(\({M_{\a_{Z\(m+m'\)}}}^TM_{\a_{Z\(m+m'\)}}\)^{k}\)\].
\end{aligned}
\end{equation}

%%%%%%%%%%%%%%%%% Moments of DRD' %%%%%%%%%%%%%%%%%%%%%

\begin{proof}
    Let $A_n = {D_n}^2$, $B_n = R_n{D_n'}^2R_n^T$ and $\varphi =\trace\otimes\Ebb$. Then 
    \begin{align*}
        &\varphi\(A_nB_n\dots, A_nB_n\) 
        = \sum_{\pi\in NC(n)} \kappa_{\pi}[A_n,\dots, A_n]\cdot \varphi_{K(\pi)} [B_1,\dots, B_n] \\
        =&  \sum_{\pi\in NC(n)} \kappa_{K(\pi)}[A_n,\dots, A_n]\cdot \varphi_{\pi} [B_1,\dots, B_n] \\
        =& \sum_{\pi\in NC(n)} \prod_{V\in K(\pi)} \kappa_{\,\abs{V}}(A_n,\dots, A_n)\cdot \prod_{W\in\pi} \varphi_{\,\abs{W}} (B_1,\dots, B_n) \\
        =& \sum_{\pi\in NC(n)} \(\prod_{V\in K(\pi)} \sum_{\sigma\in NC(\abs{V})} \varphi_{\sigma}[A_n,\dots, A_n] \cdot \mu\(\sigma, 1_{\,\abs{V}}\) \)\cdot \prod_{W\in\pi} \varphi_{\,\abs{W}} (B_1,\dots, B_n) \\
        =& \sum_{\pi\in NC(n)} \(\prod_{i=1}^p \sum_{\sigma\in NC(k_i)} \varphi_{\sigma}[A_n,\dots, A_n] \cdot \prod_{j=1}^{r_i} (-1)^{y_j-1} C_{y_j-1}\) \)\cdot \prod_{W\in\pi} \varphi_{\,\abs{W}} (B_1,\dots, B_n) \\
        =& \sum_{\substack{\pi,\sigma\in NC(n): \pi\cup \sigma\in NC(2n)}} \(\prod_{i=1}^R (-1)^{x_i-1} C_{x_i-1}\) \)\cdot \prod_{V\in \sigma} \varphi_{\,\abs{V}} (A_n,\dots, A_n) \cdot \prod_{W\in\pi} \varphi_{\,\abs{W}} (B_1,\dots, B_n) \\
    \end{align*}
\end{proof}

\begin{thm}
\begin{equation}
    \lim_{n\to\infty} \dfrac{\,1\,}{n}\cdot \Ebb\[\trace\(\(MM^T\)^k\)\] = \sum_{\substack{\pi,\sigma\in NC(n):\\ \pi\cup \sigma\in NC(2n)}} \(\prod_{i=1}^{R} (-1)^{x_i-1}C_{x_i-1}\) \cdot \o_{\pi} \o'_{\sigma}
\end{equation}
where $\o_{\pi} = \o_{2\,\abs{V_1}}\dots \o_{2\,\abs{V_r}}$ if $\pi=\{V_1,\dots, V_r\}$ and $\pi\cup\sigma$ partitions $[2n]$ into parts of sizes $\{x_1,\dots, x_R\}$.
\end{thm}

\begin{rmk}
    By the above proposition, to prove \Cref{thm:main-1}, it suffices to prove that for all $\vaa, \vbb\in P_k$,
\begin{align*}
    C\(\vaa, \vbb\) 
    &:= \lim_{n\to\infty}\dfrac{\,1\,}{n}\cdot\(\sum_{\substack{ \vi,\,\vj\subseteq [n]^k: \\ P(\,\vi\,)=\vaa,\, P(\,\vj\,)=\vbb}}
    \Ebb\[\,\prod_{m=1}^k R(i_{m},j_{m})R(i_{m+1},j_{m})\]\)\\
    %&= (-1)^{k+a+b-1}\cdot \(\dfrac{a!}{\a_1!\dots\a_k!}\)\cdot\(\dfrac{b!}{\b_1!\dots\b_k!}\)\cdot\dfrac{k}{ab}\cdot{a+b-2\choose k-1}\;.
    &= (-1)^{k+a+b-1}\cdot k\cdot \binom{a+b-2}{k-1} \cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \dfrac{(b-1)!}{\b_1!\dots\b_k!}\,.
\end{align*}
\end{rmk}


%%%%%%%%%%%%%%%%%%% C(w2^k, w2'^k) Case %%%%%%%%%%%%%%%%%%%
{\color{blue} (Old version, has some discrepancy) We will define $\E_1,\dots,\E_k$ inductively backwards starting from $\E_k$. Note that $\E_j$ is a function of $\vvv_1,\ldots,\vvv_{j-1}$
    \begin{enumerate}[i.]
        \item We define $\displaystyle \E_k=\underset{\vvv_k\in S^{n-k}}{\Ebb}\[\<\vvv_k,\ve_k^{\;\perp\times (k-1)}\>\<\vvv_k,\ve_{1}^{\;\perp\times (k-1)}\>\]$ where $\ve^{\;\perp\times i}$ is the orthogonal projection of $\ve$ onto the orthogonal complement of $\spann\(\vvv_1,\dots,\vvv_i\)$, and
            
        \item for each $i\in[k-1]$, $\displaystyle \E_i=\underset{\vvv_i\in S^{n-i}}{\Ebb}\[\<\vvv_i,\ve_i^{\;\perp\times (i-1)}\>\<\vvv_i,\ve_{i+1}^{\;\perp\times (i-1)}\>\cdot  \E_{i+1}\]$
    \end{enumerate} 
        
    Defined this way, $\E_1 = \val(G_k)$.
    
    Since 
    \begin{align*}
        \ve^{\;\perp\times i} 
        = \ve^{\;\perp\times (i-1)}-\<\vvv_{i},\ve^{\;\perp\times (i-1)}\>\cdot \vvv_{i}\,,
    \end{align*}
    
    we have that 
    \begin{align*}
        \E_k
        &= \underset{\vvv_k\in S^{n-k}}{\Ebb}\[\<\vvv_k,\ve_k^{\;\perp\times (k-1)}\>\<\vvv_k,\ve_{1}^{\;\perp\times (k-1)}\>\]\\
        &= \dfrac{1}{n-k+1} \cdot \<\,\ve_k^{\;\perp\times (k-1)}, \ve_{1}^{\;\perp\times (k-1)}\,\> \\
        &=\dfrac{1}{n-k+1} \cdot\(\<\,\ve_k^{\;\perp\times (k-2)}, \ve_{1}^{\;\perp\times (k-2)}\,\> - \<\vvv_{k-1}, \ve_k^{\;\perp\times(k-2)}\>\<\vvv_{k-1},\ve_1^{\;\perp\times(k-2)}\> \)\\
        &= -\dfrac{1}{n-k+1}\cdot \(\sum_{i=1}^{k-1} \<\vvv_i, \ve_k^{\;\perp\times(i-1)}\>\<\vvv_i,\ve_1^{\;\perp\times(i-1)}\>\)
    \end{align*}
    
    Thus
    \begin{align*}
        \E_1
        &=\dfrac{-1}{n-k+1}\(\;\Ebb\[\vvv_k\sim \vvv_1\]+\Ebb\[\vvv_k\sim \vvv_2\]+\dots+\Ebb\[\vvv_k\sim \vvv_{k-1}\]\;\)\\
        &\\
        &\sim -n^{-1}\cdot \(\val\(G_1,G_{k-1}\)+\val\(G_2,G_{k-2}\) + \dots + \val\(G_{k-1},G_1\)\) \\
        &\sim -n^{-1}\cdot \(\sum_{i=1}^{k-1} \((-1)^{i-1}\cdot  n^{-2i+1} \cdot C_{i-1}\) \cdot \( (-1)^{k-i-1}\cdot  n^{-2(k-i)+1} \cdot C_{k-i-1}\)\)\\
        &= (-1)^{k-1}\cdot n^{-2k+1}\cdot\(\sum_{i=1}^{k-1} C_{i-1}C_{k-i-1}\) \\
        &=(-1)^{k-1}\cdot n^{-2k+1}\cdot C_{k-1} \,.
    \end{align*}
     where $\vvv_k\sim \vvv_i$ means folding the $k^{th}$ row of the matrix to the $i^{th}$ row. See figure \cref{fig:grid-combine-pf} for illustration.
    }


%%%%%%%%%%%%%%%%% C(vaa, w2^k) Case %%%%%%%%%%%%%%%%%%%

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.35]{images/np-poly-contract.png}
    \caption{Illustration of \Cref{prop:noncross-partition-cycles} and \Cref{defn:np-cycle-size-Sp}: $\C_8/\P = \C_{8,1}\cup \C_{8,2}\cup \C_{8,3}\cup \C_{8,4}$ where $\P = \left\{\{2\},\{4\},\{6\},\{1,3\}, \{5,7,8\}\right\}$. Here $S_{\P}=\{1,2,3,2\}$.}
    \label{fig:np-poly-contract}
\end{figure}

\begin{prop}\label{prop:noncross-partition-cycles}
    Let $\vaa=\(\a_1,\dots,\a_k\)\in P_k$ and  $\P\in\np(\vaa)$. Then $\C_k/\P$ is a union of cycles $\C_{k,1},\dots,\C_{k,p}$ where
    \begin{enumerate}
        \item $\abs{V\(\C_{k,i}\)\cap V\(\C_{k,i+1}\)} = 1$ for each  $i\in[p-1]$.
        \item $\displaystyle p = \a_2+2\a_3+\dots+(k-1)\a_k + 1 = k-a+1$.
        \item $\displaystyle\sum_{i=1}^{p}\, \abs{\C_{k,i}} = k$.
    \end{enumerate} 
\end{prop}

\begin{defn}\label{defn:np-cycle-size-Sp}
    Let $\P$ be a non-crossing partition of $[k]$. Assume $\C_k/\P = \C_{k,1}\cup\dots\cup \C_{k,p}$. We define $S_{\P}$ to be the unordered sequence $\lcurb i_1,\dots,i_p\rcurb$ where $i_j$ is the size of the cycle $\C_{k,j}$ for each $j\in[p]$.
\end{defn}

\begin{prop}\label{prop:sum-of-xi-ni}
Let $\X=\{x_1,\dots,x_p\}$ be such that $x_1+\dots+x_p=k$. Let $s\geq 1$. Given $\(i_1,\dots,i_s\)\subseteq [p]^s$, define $\product_{\X}\(i_1,\dots,i_s\)$ as
\begin{equation*}
    \product_{\X}\(i_1,\dots,i_s\) = \prod_{j=1}^s\, \(x_{i_j}-n\(\vi, j\)\) \text{ where } n\(\vi, j\) = \abs{\lcurb m\leq j: i_m=i_j \rcurb}
\end{equation*}
Then 
\begin{align*}
    \sum_{\(i_1,\dots,i_s\)\subseteq [p]^s} \product_{\X}\(i_1,\dots, i_s\) = \(k-p\)\cdot\dots\cdot\(k-p-(s-1)\)
\end{align*}
\end{prop}

\begin{eg}
    $\displaystyle\product_{\X}\(1,2,3,1,3,3\) = (x_1-1)(x_2-1)(x_3-1)(x_1-2)(x_3-2)(x_3-3)$.
\end{eg}

\begin{proof}
    We will prove by induction on $s$.
    \begin{enumerate}
        \item Base case $s=1$: this is the same as $\displaystyle\sum_{i=1}^p\, x_i-1 = \(\sum_{i=1}^p x_i\) - p = k-p$.
        \item Inductive case $s\implies s+1$: Let $\vi=\(i_1,\dots,i_{s+1}\)$. $\product_{\X}(i_1,\dots,i_{s+1}) = \product_{\X}(i_1,\dots,i_s)\cdot \(x_{i_{s+1}}-n\(\vi,s+1\)\)$. Then
        \begin{align*}
            \sum_{\(i_1,\dots,i_{s+1}\)\subseteq [p]^{s+1}}\, \product_{\X}\(i_1,\dots, i_{s+1}\) 
            &= \sum_{\(i_1,\dots,i_s\)\subseteq [p]^s}\sum_{i_{s+1}\in[p]}\, \product_{\X}\(i_1,\dots, i_s\)\cdot \(x_{i_{s+1}}-n\(\vi,s+1\)\)\\
            &= \sum_{\(i_1,\dots,i_s\)\subseteq [p]^s}\product_{\X}\(i_1,\dots, i_s\)\cdot \(\sum_{j=1}^{p}\, x_j - \abs{\lcurb m\leq s: i_m= j\rcurb }-1\)\\
            &= \sum_{\(i_1,\dots,i_s\)\subseteq [p]^s}\product_{\X}\(i_1,\dots, i_s\)\cdot\( k - \(\sum_{j=1}^{p}\, \abs{\lcurb m\leq s: i_m= j\rcurb}\) - p\)\\
            &= \sum_{\(i_1,\dots,i_s\)\subseteq [p]^s}\product_{\X}\(i_1,\dots, i_s\)\cdot\( k - s - p\)\\
            &= \(k-p\)\cdot\dots\cdot\(k-p-(s-1)\)\cdot\(k-p-s\).
        \end{align*}
    \end{enumerate}
\end{proof}


\begin{proof}[Proof sketch]
    Let $s'=m-2$ and $s=m-1$. Let $\(i_1,\dots,i_{s'}\)\in [p]^{s'}$. We will show that for each configuration of the $\vaa'$-polygons on $\C_k$ corresponding to $\product_{\X}\(i_1,\dots,i_{s'}\)$, it can be uniquely expanded to configurations of the $\vaa$-polygons on $\C_k$ corresponding to $\product_{\X}\(i_1,\dots,i_{s'},j\)$ for each $j\in[p]$. Since
    \begin{align*}
        \sum_{j=1}^p \product_{\X}\(i_1,\dots,i_{s'},j\)
        &= \sum_{j=1}^p \product_{\X}\(i_1,\dots,i_{s'}\)\cdot\(x_j-\abs{\lcurb m\leq s': i_m=j\rcurb}-1\)\\
        &= \product_{\X}\(i_1,\dots,i_{s'}\)\cdot \(\sum_{j=1}^p x_j-\abs{\lcurb m\leq s': i_m=j\rcurb}-1\)\\
        &= \product_{\X}\(i_1,\dots,i_{s'}\)\cdot \(k-s'-p\)\\
        &=\product_{\X}\(i_1,\dots,i_{s'}\)\cdot\(k-(m-2)-\(k-\a_1-m+1\)\)\\
        &= \product_{\X}\(i_1,\dots,i_{s'}\)\cdot\(\a_1+1\)\,.
    \end{align*}
    We can conclude that 
    \begin{align*}
        \nnpl\(\vaa,\X\) = \(\a_1+1\)\cdot \nnpl\(\vaa',\X\)\,.
    \end{align*}
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:num-of-partitions-1}]
    We have $\o_2^{\,\a_1}\dots\o_{2k}^{\,\a_k}$. Rewrite it as $\o_2^{\,\a_1}\o_{2t_1}\dots\o_{2t_m}$ where $m=\a_2+\dots+\a_k$ and treat all $t_i$'s as distinct for now. Then by Corollary \ref{cor:num-of-partitions-multipoly}, $\N\P\P\(\o_2^{\,\a_1}\o_{2t_1}\dots\o_{2t_m},\X\) = \dfrac{(a-1)!}{\a_1!}\cdot k\cdot (k-a)!$. Since there are $\a_i$ many $\o_i$ terms for $i=2,\dots,k$, to take care of the double counting we need to divide the counting by $\a_2!\a_3!\dots\a_k!$, thus
    \begin{align*}
        \nnp\(\vaa,\X\) 
        &= \dfrac{(a-1)!}{\a_1!}\cdot k\cdot (k-a)!\cdot\dfrac{1}{\a_2!\dots\a_k!}
        = \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot k\cdot (k-a)! \\
        &= \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot k\cdot (p-1)!
    \end{align*}
    as wanted.
\end{proof}

%%%%%%%%%%%%%%%%% C(vaa,vbb) General Case %%%%%%%%%%%%%%%%%
\begin{tcolorbox}[colback=white]
    {\bfseries\boldmath$\displaystyle\Omega_2^n\Omega_{2(k-n)}\cdot\Omega_2'^m\Omega'_{2(k-m)}$}, when $m,n\leq k-2$: $\displaystyle C\(\vec{\a}, \vec{\b}\) = k\cdot{m+n\choose k-1}$.
\end{tcolorbox}

\begin{tcolorbox}[colback=white]
    $\displaystyle C\(\vaa, \vbb\) = (-1)^{a+b-k-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot\dfrac{(b-1)!}{\b_1!\dots\b_k!}\cdot k\cdot{a+b-2\choose k-1}$ where $a=\a_1+\dots+\a_k$ and $b=\b_1+\dots+\b_k$.
\end{tcolorbox}

\begin{thm}[{\bf\color{blue} Delete later}]
    \begin{equation}
        C\(\o_2^{n}\,\o_{2(k-n)},\, \Omega_2'^{m}\,\o_{2(k-m)}\)=(-1)^{k+n+m+1}\cdot k\cdot {m+n\choose k-1}\,.
    \end{equation}
\end{thm}
\begin{proof}
$\Omega_2^n\,\Omega_{2(k-n)}$ squeeze $k-n$ rows, break the grid into $k-n$ parts. $\Omega_2'^m\Omega'_{2(k-m)}$ then selects one of the $k-n$ parts and squeeze $k-m$ columns of it, breaking the selected part further into $k-m$ parts.

Let $s=(k-n-1)+(k-m)=2k-(m+n+1)$ be the total number of parts $\(\Omega_2^n\Omega_{2(k-n)}\)\(\Omega_2'^m\Omega'_{2(k-m)}\)$ breaks the grid into. Let $i_1,\dots,i_{k-n-1},i'_{k-n}$ denotes the size of the parts $\Omega_2^n\Omega_{2(k-n)}$ breaks the grid into where $i'_{k-n}$ is the part $\Omega_2'^m\Omega'_{2(k-m)}$ will select. Let $i_{k-n},\dots,i_s$ be the size of the parts $\Omega_2'^m\Omega'_{2(k-m)}$ breaks $i'_{k-n}$ into.

Note $i'_{k-n}=k-(i_1+\dots+i_{k-n-1})$. $i_{k-n}+\dots+i_s=i'_{k-n}$. $i_1+\dots+i_s=k$.

\begin{equation*}
\begin{aligned}
    & k\cdot\sum_{i_1=1}^{k}\sum_{i_2=1}^{k-i_1}\dots\sum_{i_{k-n-1}=1}^{k-i_1-\dots-i_{k-n-2}} C_{i_1-1}\cdot\dots\cdot C_{i_{k-n-1}-1}\cdot\(\sum_{i_{k-n}+\dots+i_s=i'_{k-n}}  \dfrac{i'_{k-n}}{k-m}\cdot C_{i_{k-n}-1}\cdots C_{i_s-1}\)\\
    &= \dfrac{k^2}{k-m}\(\sum_{i_1+\dots+i_s=k} C_{i_1-1}\dots C_{i_s-1}\) -\dfrac{k(k-n-1)}{k-m}\(\sum_{i_1+\dots+i_s=k}i_1\cdot C_{i_1-1}\dots C_{i_s-1}\)\\
    &= \(\dfrac{k^2}{k-m}-\dfrac{k(k-n-1)}{k-m}\cdot\dfrac{k}{s}\)\cdot\(\sum_{i_1+\dots+i_s=k} C_{i_1-1}\dots C_{i_s-1}\) \\
    &=\(\dfrac{k^2(s-k+n+1)}{(k-m)s}\)\cdot\(\sum_{i_1+\dots+i_s=k} C_{i_1-1}\dots C_{i_s-1}\)\\
    &= \dfrac{k^2}{s}\cdot\(\sum_{i_1+\dots+i_s=k} C_{i_1-1}\dots C_{i_s-1}\)
     = \dfrac{k^2}{s}\cdot s\cdot\dfrac{(2k-s-1)!}{(k-s)!k!}
     = k\cdot{m+n\choose k-1}.
\end{aligned}
\end{equation*}

\end{proof}

%%%%%%%%%%%%%%%%%% Section 4: Z(m)+\o %%%%%%%%%%%%%%%%%%%%

= \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\({\mzshapeo}^T\mzshapeo\)^{k}\)\] }

Recall that $\np\(\vaa\)$ is the set of noncrossing partitions of $[k]$ such that there are $\a_i$ many parts of size $i$. We have the following result from the paper \cite{liaw1998simple}.

\begin{thm}\label{thm:num-of-np}
    Let $\vaa\in P_k$. Then 
    \begin{equation}
        \abs{\np\(\vaa\)} = {k\choose a-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!}\,.
    \end{equation}
\end{thm}

\begin{defn}
    Given $\vaa\in P_k$, we define $\np\(m\vaa\)$ to be the set of noncrossing partitions of $[mk]$ corresponding to augmented $\vaa$: there are $\a_i$ parts of size $mi$ in a partition $P\in\np\(m\vaa\)$.
\end{defn}

A direct Corollary is the following.
\begin{cor}\label{cor:num-of-m*np}
    Let $\vaa\in P_k$. Then 
    \begin{equation}
        \abs{\np\(m\vaa\)} = {mk\choose a-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!}\,.
    \end{equation}
\end{cor}
\begin{proof}
    This is an application of Theorem \ref{thm:num-of-np}. Since $\np\(m\vaa\)$ is the set of non-crossing partitions of $[mk]$ with $a$ parts, and there are $\a_i$ number of parts with size $mi$, $\displaystyle\abs{\np\(m\vaa\)}={mk\choose a-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}$ as wanted.
\end{proof}

\begin{cor}\label{cor:m-catalan-nnp}
Let $\vaa = \(k,0,\dots,0\)\in P_k$. Then
\begin{equation}
    C(k,m) = \abs{\np\((m+1)\vaa\)}
\end{equation}

i.e. $C(k,m)$ is the number of non-crossing partitions of $[(m+1)k]$ where all the parts are of size $(m+1)$.
\end{cor}
\begin{proof}
    %The set of non-crossing partitions of $[(m+1)k]$ where all the parts are of size $(m+1)$ corresponds to $\np\((m+1)\vaa\)$ where $\vaa = \(k,0,\dots,0\)$. 
    By Corollary \ref{cor:num-of-m*np},
    \begin{align*}
        \abs{\np\((m+1)\vaa\)} 
        &= {(m+1)k\choose k-1}\cdot\dfrac{(k-1)!}{k!}
         = \dfrac{\((m+1)k\)!}{(k-1)!(mk+1)!}\cdot\dfrac{\,1\,}{k}
         = \dfrac{\((m+1)k\)!}{k!(mk)!}\cdot\dfrac{1}{mk+1}\\
        &= {(m+1)k\choose k}\cdot\dfrac{1}{mk+1} = C(k,m).
    \end{align*}
    as wanted.
\end{proof}


consider the random matrix $\mmzshape = D'RD$ where $\o'=\ozm$ and $\o=\ozmm$.

\begin{thm}
Let $\mmzshape$ be defined as above. Then
\begin{equation}
    \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\({\mmzshape}^T\mmzshape\)^{k}\)\] = C\(k,m+m'\)\,.
\end{equation}
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Section 5: M_{Z(m),s} %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thm}
    Let $M_{\mzshape}$ be the $Z(m)$-shape graph matrix. Let $\displaystyle M_{n,m} = \dfrac{1}{n^{m/2}} M_{\mzshape}$ and $\displaystyle r(n,m) = \dfrac{n!}{(n-m)!}$. Then 
    \begin{equation}
        \lim_{n\to\infty} \dfrac{1}{r(n,m)}\cdot \Ebb\[\trace\(\(M_{\mzshape}M_{\mzshape}^T\)^k\)\] = C(k,m)
    \end{equation}
    for all $k\in\Nbb$.
\end{thm}

Consider the random matrix $M_{Z(m),s}$ obtained inductively on distributions $\o^{(1)},\dots,\o^{(s)}$ as the following:
\begin{enumerate}
    \item $M_{Z(m),0} = M_{\a_{Z(m)}}$ is the $Z(m)$-shape graph matrix.
    \item $M_{Z(m),1} = D'RD$ where $\o'=$ the singular value distribution of $M_{m,0}$ and $\o=\o_1$. i.e. $\o_{2i}' = C(i,m)$ for all $i$.
    \item $M_{Z(m),s} = D'RD$ where $\o'=$ the singular value distribution of $M_{Z(m),s-1}$ and $\o=\o^{(s)}$.
\end{enumerate}

\begin{defn}
    We will denote $C_m\(\vaa_1,\dots,\vaa_s\)$ to be 
    \begin{equation}
        C_m\(\vaa_1,\dots,\vaa_s\) = {(m-s+1)k\choose mk - (a_1+\dots+a_s) + 1}\cdot k^{s-1}\cdot \prod_{i=1}^s \dfrac{(a_i-1)!}{\a_{i1}!\dots\a_{ik}!}
    \end{equation}
    
    Then Theorem \ref{thm:expression-for-mzshape-sdistr} can be rewritten as 
    \begin{equation}
        A_{m}^{(s)}\(k,\underbrace{0,\dots,0}_{s}\) = \sum_{\vaa_i\in P_k}\, C_m\(\vaa_1,\dots,\vaa_s\)\cdot \prod_{i=1}^s\, \vv{\o^{(i)}}^{\vaa_i}
    \end{equation}
\end{defn}

let $\mzshapesdistr$ be defined as above. Then
\begin{equation}
     \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\mzshapesdistr\mzshapesdistr^T\)^{k}\)\]
    = \sum_{\vaa_i\in P_k}\, C_m\(\vaa_1,\dots,\vaa_s\)\cdot \vv{\o^{(1)}}^{\,\vaa_1}\dots \vv{\o^{(s)}}^{\,\vaa_s}
\end{equation}

{\color{blue} or the following...?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% Section 6: Recur %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The following theorem states the recurrence relation for $A_2(k,r)$.
\begin{thm}\label{thm:recur-grid-base-z}
\begin{equation}
    A_2\(k,r\) 
    = \sum_{\substack{i_1,i_2,i_3\geq 0: \\ i_1+i_2+i_3 = k-1}}\, A_2\(i_1,0\)\cdot A_2\(i_2,0\)\cdot A_2\(i_3,r+1\)\,
\end{equation}
and 
\begin{equation}
    A_2(0,r) = \o_{2r}\,.
\end{equation}
\end{thm}

Before proving \Cref{thm:recur-grid-base-Z}, we prove a simpler version, when $m=1$ instead of $2$, and then generalize the proof to $m=2$.

Apply Corollary \ref{cor:expected-trace-for-bipartite-shapes} to $\mzshapesdistrg$, we get the following result.
\begin{cor}
Let $\oa=\o_{\mzshape,s}$ be as in Definition \ref{defn:mzshape-sdistr-graph-matrix}. Let $\displaystyle r(n,m)=\dfrac{n!}{(n-m)!}$. Then
    \begin{equation}
        \lim_{n \to \infty} {\dfrac{1}{r(n,m)}\cdot \Ebb\[\trace\(\(\mzshapesdistrg{\mzshapesdistrg}^T\)^q\)\]} = W\(\D_{\mzshape,\oa,2q}\)
    \end{equation}
\end{cor}

\begin{proof}
Let $\a = \mzshape$. Then $s_{\a} = m$, $\displaystyle r_{approx}(n) = \dfrac{n!}{(n-m)!}$, and $n^{\abs{V(\a)-s_{\a}}} = n^{m}$. Thus $\displaystyle \dfrac{M_{\a,\oa}{M_{\a,\oa}}^T}{n^{|V(\a)| - s_{\a}}} = \dfrac{M_{\a,\oa}{M_{\a,\oa}}^T}{n^{m}} = \(\dfrac{M_{\mzshape,s}}{n^{m/2}}\)\(\dfrac{M_{\mzshape,s}}{n^{m/2}}\)^T = \mzshapesdistrg{\mzshapesdistrg}^T$. Plug these into Corollary \ref{cor:expected-trace-for-bipartite-shapes} we get the above statement.
\end{proof}

\begin{defn}\label{defn:Ams}
{\color{blue}\bfseries\boldmath Note: not correct for the $s>1$ case.}

    We define $A_m^{(s)}\(k,r_1,\dots,r_s\)$ to be
    \begin{align}
        \sum_{\vaa_i\in P_{k}} \sum_{i_1=1}^k\dots\sum_{i_s=1}^k \,  C_m\(\vaa_1,\dots,\vaa_s\)\cdot \(\prod_{j=1}^s \dfrac{i_j\cdot\a_{j,i_j}}{k} \cdot \vv{\o^{(j)}}^{\vaa_j}\(i_j,+r_j\)\)
    \end{align}
\end{defn}

\begin{rmk}
    When $s=1$, denote $A_m^{(s)}\(k,r_1,\dots,r_s\)$ as $A_m\(k,r\)$. Then 
    \begin{equation}
        A_m\(k,r\) = \sum_{\vaa\in P_k}\, \sum_{\substack{\P=\{P_1,\dots,P_a\}in \\ \np(m\vaa):\, 1\in P_1 }}\,  \(\o_{2\,\(|P_1|/m+r\)}\o_{2\,|P_2|/m} \cdot\dots\cdot \o_{2\,|P_a|/m}\)
    \end{equation}
    
    Moreover, when $m=1$, denote $A_m\(k,r\)$ as $A\(k,r\)$. Then
    \begin{equation}
        A\(k,r\) = \sum_{\vaa\in P_k}\, \sum_{\substack{\P=\{P_1,\dots,P_a\}in \\ \np(\vaa):\, 1\in P_1 }}\,  \(\o_{2\,\(|P_1|+r\)}\o_{2\,|P_2|} \cdot\dots\cdot \o_{2\,|P_a|}\)
    \end{equation}
\end{rmk}

\begin{prop}\label{prop:Akr}
{\color{blue} \bfseries Note: Don't need this with the new definition.}
\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.32]{images/np-expand.png}
    \caption{Illustration of \Cref{prop:Akr}: first row is $A(3,0)$, second row is $A(3,1)$.}
    \label{fig:np-expand}
\end{figure}

    \begin{equation}
        A(k,0) = \sum_{\P = \{P_1,\dots,P_a\}\in\np_k}\, \o_{2\,\abs{P_1}}\cdot\dots\cdot \o_{2\,\abs{P_a}}\,.
    \end{equation}
    and 
    \begin{equation}
        A(k,r) = \sum_{\substack{\P = \{P_1,\dots,P_a\}\in\np_k:\\ 1\in P_1}}\, \o_{2\,\(\abs{P_1}+r\)} \o_{2\,\abs{P_2}}\cdot\dots \cdot \o_{2\,\abs{P_a}}\,.
    \end{equation}
\end{prop}

\begin{proof}
    By \Cref{thm:num-of-np}, $\displaystyle {k\choose a-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!} = \abs{\np\(\vaa\)}$. Thus
    \begin{align*}
        A(k,0) 
        &= \sum_{\vaa\in P_k} {k\choose a-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \voo^{\vaa}
        = \sum_{\vaa\in P_k} \abs{\np\(\vaa\)}\cdot \voo^{\vaa}\\
        &=\sum_{\vaa\in P_k}\; \sum_{\P = \{P_1,\dots,P_a\}\in\np(\vaa)}\, \o_{2\,\abs{P_1}}\cdot\dots\cdot \o_{2\,\abs{P_a}}\, \\
        &= \sum_{\P = \{P_1,\dots,P_a\}\in\np_k}\, \o_{2\,\abs{P_1}}\cdot\dots\cdot \o_{2\,\abs{P_a}}\,.
    \end{align*}
\end{proof}

When $m=1, s=1$, we have that
\begin{equation}
    A(k,0) = \(\o_{Z(1)}\opr \o\)_{2k} = \(\o_{\a_0}\opr \o\)_{2k} = \sum_{\vaa\in P_k} {k\choose a-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \voo^{\vaa}\,.
\end{equation}
and 
\begin{equation}
    A(k,r) = \sum_{\vaa\in P_{k}} {k\choose a-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \( \sum_{i=1}^k \, \dfrac{i\cdot\a_{i}}{k} \cdot \voo^{\vaa}\(i,+r\)\)
\end{equation}

\begin{align}
    A_m^{(s)}\(k,r_1,\dots,r_s\) = \sum_{\vaa_i\in P_{k}} \sum_{i_1=1}^k\dots\sum_{i_s=1}^k \,  C_m\(\vaa_1,\dots,\vaa_s\)\cdot \(\prod_{j=1}^s \dfrac{i_j\cdot\a_{j,i_j}}{k} \cdot \vv{\o^{(j)}}^{\vaa_j}\(i_j,+r_j\)\)
\end{align}

\begin{prop}
{\color{blue} \bfseries Note: Don't need this with the new definition.}
    \begin{equation}
        A_m(k,0) = \sum_{\vaa\in P_k}\; \sum_{\substack{\P = \{P_1,\dots,P_a\}\\ \in\np(m\vaa)}}\, \o_{2\,\abs{P_1}/m}\cdot\dots\cdot \o_{2\,\abs{P_a}/m}\,.
    \end{equation}
    and 
    \begin{equation}
        A_m(k,r) =\sum_{\vaa\in P_k}\; \sum_{\substack{\P = \{P_1,\dots,P_a\}\\ \in\np(m\vaa):\, 1\in P_1}}\, \o_{2\,\(\abs{P_1}/m+r\)} \o_{2\,\abs{P_2}/m}\cdot\dots \cdot \o_{2\,\abs{P_a}/m}\,.
    \end{equation}
\end{prop}

\begin{proof}
    By \Cref{cor:num-of-m*np}, $\displaystyle {mk\choose a-1}\cdot\dfrac{(a-1)!}{\a_1!\dots\a_k!} = \abs{\np\(m\vaa\)}$. Thus
    \begin{align*}
        A(k,0) 
        &= \sum_{\vaa\in P_k} {mk\choose a-1}\cdot \dfrac{(a-1)!}{\a_1!\dots\a_k!}\cdot \voo^{\vaa}
        = \sum_{\vaa\in P_k} \abs{\np\(m\vaa\)}\cdot \voo^{\vaa}\\
        &= \sum_{\vaa\in P_k}\; \sum_{\P = \{P_1,\dots,P_a\}\in\np(m\vaa)}\, \o_{2\,\abs{P_1}/m}\cdot\dots\cdot \o_{2\,\abs{P_a}/m}\,\\
        &= \sum_{\substack{\P = \{P_1,\dots,P_a\}\in\np_{mk}: \\ \abs{P_j} = m\cdot i_j \text{ for } j\in[a]\\ }}\, \o_{2i_1}\cdot\dots\cdot \o_{2i_a}
    \end{align*}
\end{proof}

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[t]{.55\textwidth}
        \includegraphics[width=1\linewidth]{images/recur-grid-base-2.png}
        \caption{}
        \label{fig:sdf}
    \end{subfigure}
    \begin{subfigure}[t]{.44\textwidth}
        \includegraphics[width=1\linewidth]{images/recur-grid-base-m.png}
        \caption{}
        \label{fig:fd}
    \end{subfigure}
    \caption{{\color{blue} Too small? }}
    \label{fig:dfs}
\end{figure}

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[t]{.48\textwidth}
        \includegraphics[width=1\linewidth]{images/recur-grid-general-1.png}
        \label{fig:recur-grid-general-left}
    \end{subfigure}
    \begin{subfigure}[t]{.48\textwidth}
        \includegraphics[width=1\linewidth]{images/recur-grid-general-2.png}
        \label{fig:recur-grid-general-right}
    \end{subfigure}
    \caption{Illustration of the proof of \Cref{thm:recur-grid-general}: Here $s=3$, $m=4$, $\mh=m-s+1=2$ and $k=8$. In the clockwise direction, $v_{3,7}$ is the first vertex in the same partition set as $v_{3,1}$, and $v_{2,6}$ is the first vertex in the same partition set as $v_{2,7}$. The resulting orange and blue shaded parts correspond to $A_4^{(3)}(k_3,0,0,r_3+1)$ and $A_4^{(3)}(k_2,0,r_2+1,0)$, respectively, where $k_3=2$, $k_2=1$. $v_{1,5}$ and $v_{1,8}$ are the first two vertices in the same partition set as $v_{1,12}$ in the clockwise direction, thus $t_1=2, t_2=3$. The white middle part and the green shaded part correspond to $A_4^{(3)}(q_1,0,0,0)$ and $A_4^{(3)}(q_2,0,0,0)$, respectively, where $q_1=q_2=1$. The last cycle corresponds to $A_4^{(3)}(j_2-t_2-1,r_1+1,0,0)$ where $j_2-t_2-1 = 6-3-1 = 2$.}
    \label{fig:recur-grid-general}
\end{figure}


%%%%%%%%%%%%%% Section 6 - Graph Matrices %%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:line-shape-first-constrained-vertex}
    Let $C \in \C_{(\a_0,2q)}$ be a dominant constraint graph. If $i_j$ is the first vertex $i_1$ is constrained to (i.e. if $j$ is the smallest index such that $i_1\=i_j$), then $i_2\=i_{j-1}$.
\end{lemma}

\begin{defn}
    Given $\o$, we define $B\(k,0\)$ to be 
    \begin{equation}
        B\(k,0\) = W\(\D_{\zshape,\o_{\zshape,1},2k}\)\,.
    \end{equation}
\end{defn}

\begin{defn}
    We define $B\(k,r\)$ to be the weight of dominant constraint graphs of length $k$ associated with $\zshape$ and $\o_{\zshape,1}$ where the first spoke on the first layer has an multi-edge of multiplicity $(2r+1)$.
\end{defn}

\begin{defn}
Given $\o$, we define $B_{m}\(k,0\)$ to be 
\begin{equation}
    B_{m}\(k,0\) = W\(\D_{\mzshape,\o_{\mzshape,1},2k}\)\,.
\end{equation}
\end{defn}

\begin{defn}
    We define $B_{m}\(k,r\)$ to be the weight of dominant constraint graphs of length $k$ associated with $\a_{Z(m)}$ and $\o_{\mzshape,1}$ where the first spoke on the first layer has an multi-edge of multiplicity $(2r+1)$.
\end{defn}

\begin{defn}
Given $\o^{(1)},\dots,\o^{(s)}$, we define $B_{m}^{(s)}\(k,0,\dots,0\)$ to be 
\begin{equation}
    B_{m}^{(s)}\(k,0,\dots,0\) = W\(\D_{\mzshape,\o_{\mzshape,s},2k}\)\,.
\end{equation}
\end{defn}

\begin{defn}
    We define $B_{m}^{(s)}\(k,r_1,\dots,r_s\)$ to be the weight of dominant constraint graphs of length $k$ associated with $\a_{Z(m)}$ and $\o_{\mzshape,s}$ where the first spoke on the $i^{th}$ layer has multi-edge of multiplicity $(2r_i+1)$ for $i=1,\dots, s$.
\end{defn}

\begin{thm}\label{thm:recur-relation-mzshape-sdistr-graph}
\begin{equation}
\begin{aligned}
    B_{m}^{(s)}\(k,r_1,\dots,r_s\) 
    = \sum_{\substack{i_1,\dots,i_{m+1}\geq 0: \\ i_1+\dots+i_{m+1} = k-1}}\, & B_{m}^{(s)}\(i_1,r_1+1,0,\dots,0\)\dots B_{m}^{(s)}\(i_s,0,\dots,0,r_s+1\)\cdot\\
    & B_{m}^{(s)}\(i_{s+1},0,\dots,0\)\dots B_{m}^{(s)}\(i_{m+1},0,\dots,0\)
\end{aligned}
\end{equation}
\end{thm}

\begin{cor}
$\mzshapesdistr$ and $M^{(G)}_{Z(m),s}$ has the same moments. i.e. Let $\displaystyle r(n,m)=\dfrac{n!}{(n-m)!}$, then
    \begin{equation}
        \lim_{n\to\infty}\, \dfrac{\,1\,}{n}\cdot\Ebb\[\trace\(\(\mzshapesdistr\mzshapesdistr^T\)^{k}\)\] = \lim_{n\to\infty}\, \dfrac{\,1\,}{r(n,m)}\cdot\Ebb\[\trace\(\(M^{(G)}_{Z(m),s}{M^{(G)}_{Z(m),s}}^T\)^{k}\)\] 
    \end{equation}
    for all $k\geq 0$.
\end{cor}


{\color{blue} \textbf{Previous Version}
\begin{proof}

We will prove \Cref{thm:recur-graph-zshape} in two steps:
\begin{enumerate}
    \item 
    
    \begin{figure}[hbt!]
        \centering
        \includegraphics[scale=0.3]{images/recur-z-shape-split-1.png}
        \caption{Illustration of \Cref{thm:recur-graph-zshape}, splitting step 1: The spoke $\{a_{12},b_{11}\}$, colored orange, has multiplicity $2r+1$.}
        \label{fig:z-shape-1}
    \end{figure}
    
    Let $i \in [k]$ be the first index such that $a_{12} \= a_{(i+1)2}$. In the case of $a_{12}$ being isolated, $i$ is chosen to be $k$. This implies that $b_{12} \= b_{i2}$, which further implies that $b_{11}\=b_{i1}$. Moreover, contracting $b_{11}$ and $b_{i1}$ together and contracting $b_{12}$ and $b_{i2}$ together splits $H\(\a_Z,2k\)$ into $H\(\a_Z,2(i-1)\)$ and $H\(\a_Z,2(k-i+1)\)$, and the induced constraint graphs $C' \in \C_{\(\a_Z,2(i-1)\)}$ and $C'' \in \C_{\(\a_Z,2(k-i+1)\)}$ are dominant. Now observe that 
    \begin{enumerate}[i.]
        \item Since $a_{12} \= a_{(i+1)2}$ in $C$, $a_{12} \= a_{22}$ in $C''$.
        \item If we are given dominant constraint graphs $C' \in \mathcal{C}_{\(\a_Z,2(i-1)\)}$ and $C'' \in \mathcal{C}_{\(\a_Z,2(k-i+1)\)}$ such that $a_{12} \= a_{22}$ in $C''$, we can recover $C$ and $i$ by reversing this process. Thus, this map is a bijection. 
    \end{enumerate}
    
    This implies that when $a_{12}$ is not isolated and $a_{12}\=a_{i+1,2}$, the weight of all such dominated constraint graphs is 
    \begin{equation}
        W\(\left\{C\in \B_{k-i+1,r}: a_{12}\= a_{22}\right\}\) \cdot B(i-1,0)
    \end{equation}
    
    See \Cref{fig:z-shape-1} for illustration.
    
    If $a_{12}$ is isolated then we must have that $b_{12} \= b_{k2}$. In this case, $b_{11} \= b_{k1}$ and contracting along these edges gives us $B(k-1,0)$ and ....
    
    Combining the argument together, we get
    \begin{equation}
        B(k,r) = \sum_{i=1}^k\, W\(\left\{C\in \B_{k-i+1,r}:  a_{12}\= a_{22}\right\}\) \cdot B(i-1,0).
    \end{equation}
    
    \item 
    
    \begin{figure}[hbt!]
        \centering
        \includegraphics[scale=0.3]{images/recur-z-shape-split-2.png}
        \caption{Illustration of \Cref{thm:recur-graph-mzshape}, splitting step 2: The spoke $\{a_{12},b_{11}\}$, colored orange, has multiplicity $2r+1$. After the splitting, the spoke $\{a_{12},b_{11}\}$ has multiplicity $2r+3$ since $\{a_{12},b_{11}\}\longleftrightarrow\{b_{11},a_{22}\} \longleftrightarrow \{a_{j+1,2},b_{j+1,1}\}$}
        \label{fig:z-shape-2}
    \end{figure}
    
    Now we are going to prove that
    \begin{equation}
          W\(\left\{C\in \B_{k,r}:  a_{12}\= a_{22}\right\}\) = \sum_{j=1}^k B(k-j,r+1)\cdot B(j-1,0).
    \end{equation}
    
    If $b_{11}$ is not isolated, let $j\in[k-1]$ be the first index such that $b_{j+1,1} \= b_{11}$. Then this implies that $a_{21} \= a_{j+1,1}$, which further implies that $a_{22}\= a_{j+1,2}$. Contracting $a_{22}$ with $a_{j+1,2}$ and $a_{21}$ with $a_{j+1,2}$, we get $B(j-1,0)$ on the right and $B(k-j,r+1)$ on the right since $\{a_{12},b_{11}\} \= \{b_{11},a_{22}\} \= \{a_{j+1,2},b_{j+1,1}\}$. 
    
    See \Cref{fig:z-shape-2} for illustration.
    
    When $b_{11}$ is isolated, then $a_{k1}\= a_{21}$. Contracting $a_{k1}$ with $a_{21}$ and $a_{12}$ with $a_{22}$, we get $B(k-1, 0)$ and $B(0,r+1)$.
    
    Thus combining the above argument, we proved the equation.
\end{enumerate}

In conclusion, combing step 1 and 2, we conclude that 
\begin{align*}
    B(k,r) 
    &= \sum_{i=1}^{k} W\(\left\{C\in \B_{k-i+1,r}:  a_{12}\= a_{22}\right\}\)\cdot B(i-1,0) \\
    &= \sum_{i=0}^{k-1} W\(\left\{C\in \B_{k-i,r}:  a_{12}\= a_{22}\right\}\)\cdot B(i,0) \\
    &= \sum_{i=0}^{k-1} \(\sum_{j=1}^{k} B(k-i-j,r+1)\cdot B(j-1,0)\)\cdot B(i,0)\\
    &= \sum_{i=0}^{k-1} \(\sum_{j=0}^{k-1} B(k-i-j-1,r+1)\cdot B(j,0)\)\cdot B(i,0)\\
    &= \sum_{\substack{i_1,i_2,i_3\geq 0: \\ i_1+i_2+i_3 = k-1}} B(i_1,0)\cdot B(i_2,0)\cdot B(i_3,r+1).
\end{align*}

\end{proof}
}

\comm{
\begin{proof}

The proof will be similar to the proof for \Cref{thm:recur-graph-mzshape}, with the modification that some of the $B_m(i_j,0)$ in the split would become $B_m(i_j,0,\dots,r_j+1,\dots,0)$, since instead of the $\o_{\pm 1}$ distribution, now we have the $\o^{(j)}$ distribution on the spokes in the $j^{th}$ layer. 

Follow the same steps as in \Cref{thm:recur-graph-mzshape}. At the $t^{th}$ splitting step,
\begin{enumerate}
    \item if $1\leq t\leq m-s$, then we split $\big\{C\in \B_{m-t+2,k_{t-1},r_1,\dots,r_s}\cup\, \B_{t-2, k_{t-1}-1}: a_{1,m-t+2}\= a_{2,m-t+2}\big\}$ from the $(t-1)^{th}$ step into $\B_{m,i_{m-t+1}-1}$ and $\big\{C\in \B_{m-t+1,k_t,r_1,\dots,r_s}\cup\, \B_{t-1, k_t-1}: a_{1,m-t+1}\= a_{2,m-t+1}\big\}$ where $k_j=k-\(i_m+i_{m-1}+\dots+i_{m-j+1}\)+j$ for each $j\in[t]$.
    
    %we have obtained $\B_{m,i_j-1,0}$ for $j=m,m-1,\dots,m-t+1$ and $\big\{C\in \B_{m-t+1,k_t,r}\cup\, \B_{t-1, k_t-1, 0}: a_{1,m-t+1}\= a_{2,m-t+1}\big\}$ where $k_t=k-\(i_m+i_{m-1}+\dots+i_{m-t+1}+t\)$.
    
    \item if $m-s+1\leq t\leq m$, then we split $\big\{C\in \B_{m-t+2,k_{t-1},r_1,\dots,r_{m-t+1}}\cup\, \B_{t-2, k_{t-1}-1}: a_{1,m-t+2}\= a_{2,m-t+2}\big\}$ from the $(t-1)^{th}$ step into $\B_{m,i_{m-t+1}-1,(r_{m-t+1}+1)\ve_{m-t+1}}$ and $\big\{C\in \B_{m-t+1,k_t,r_1,\dots,r_{m-t}}\cup\, \B_{t-1, k_t-1}: a_{1,m-t+1}\= a_{2,m-t+1}\big\}$ where $k_j=k-\(i_m+i_{m-1}+\dots+i_{m-j+1}\)+j$ for each $j\in[t]$.
    
    When $t=m$ (the last step), $\big\{C\in \B_{m-t+1,k_t,r_1,\dots,r_{m-t}}\cup\, \B_{t-1, k_t-1}: a_{1,m-t+1}\= a_{2,m-t+1}\big\} = \B_{1,k_m}\cup\, \B_{m-1, k_m-1}: a_{11}\= a_{21}\big\} = \B_{m,k_m-1}$ where $k_m=k-\(i_m+i_{m-1}+\dots+i_{1}\)+m$.
\end{enumerate}

Thus combining everything, we have 
\begin{align*}
     &B_m(k,r) \\
    =& \sum_{i_1,\dots,i_m\geq 1} \(\prod_{j=1}^{s} B_m(i_j-1,0,\dots,r_j+1,\dots,0)\)\cdot \(\prod_{j=s+1}^{m} B_m(i_j-1,0,\dots,0)\)\cdot  B_m(k_m-1,0,\dots,0)\\
    &\hspace{2cm} \text{ where } k_m=k-\(i_m+i_{m-1}+\dots+i_{1}\)+m \\
    =& \sum_{\substack{j_1,\dots,j_{m+1}\geq 0: \\ j_1+\dots+j_{m+1} = k-1}}\, \(\prod_{j=1}^{s} B_m(i_j-1,0,\dots,r_j+1,\dots,0)\)\cdot \(\prod_{j=s+1}^{m+1} B_m(i_j-1,0,\dots,0)\)
\end{align*}
\end{proof}
as wanted.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Section 7 %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defn}[Shapes]
We define a \emph{shape} $\alpha$ to be a graph with vertices $V(\alpha)$, edges $E(\alpha)$, and distinguished tuples of vertices $U_{\alpha} = \(u_1,\ldots,u_{\abs{U_{\alpha}}}\)$ and $V_{\alpha} = \(v_1,\ldots,v_{\abs{V_{\alpha}}}\)$.
\end{defn}

\begin{defn}[Bipartite Shapes]
We say that a shape $\alpha$ is \emph{bipartite} if $U_{\alpha} \cap V_{\alpha} = \emptyset$, $V(\alpha) = U_{\alpha} \cup V_{\alpha}$, and all edges in $E(\alpha)$ are between $U_{\alpha}$ and $V_{\alpha}$.
\end{defn}

\begin{rmk}
    A shape $\a$ is associated with a set of distributions $\oa=\{\o_e:e\in E(\a)\}$, one for each edge of $\a$.
\end{rmk}

\begin{defn}[Fourier Characters]
    Given a shape $\a$ associated with distributions $\oa$, a graph $G=\(V(G),E(G)\)$ and an injective map $\sigma: V(\alpha) \to V(G)$, we define $\chi_{\sigma(E(\a))}(G) = \prod_{e \in E(\a)} x_{\sigma(e)}^{e}$ where each \textit{edge variable} $x_{\sigma(e)}^e$ is sampled independently from $\o_e$.
\end{defn}

\begin{defn}[Graph Matrices with Input Distributions $\oa$]
Given a shape $\a$ associated with distributions $\oa$, we define $M_{\alpha,\oa}$, the \emph{graph matrix with input distributions $\oa$} to be the $\frac{n!}{\(n-\abs{U_{\alpha}}\)!}\times\frac{n!}{\(n-\abs{V_{\alpha}}\)!}$ matrix with rows indexed by tuples of $\abs{U_{\alpha}}$ distinct vertices, columns indexed by tuples of $\abs{V_{\alpha}}$ distinct vertices, and entries
\begin{equation*}
    M_{\alpha,\oa}(A,B) = \sum_{\sigma: V(\alpha) \to V(G): \sigma \text{ is injective}, \atop \sigma(U_{\alpha}) = A, \sigma(V_{\alpha}) = B} \chi_{\sigma(E(\a))}(G).
\end{equation*}
\end{defn}

\begin{defn}[Graph Matrices with Single Input Distribution $\o$]
    We say a graph matrix is with single input distribution $\o$ if $\oa=\{\o\}$. i.e. $\o_e=\o$ for all $e\in E(\a)$. We denote it by $M_{\a,\o}$.
\end{defn}

\begin{defn}\label{defn:z-shape}
    Let $\a_{Z}$ be the bipartite shape with vertices $V(\a_{Z})=\{u_1,u_2,v_1,v_2\}$ and edges $E(\a_{Z})=\left\{\{u_1,v_1\},\{u_2,v_1\},\{u_2,v_2\}\right\}$ with distinguished tuples of vertices $U_{\a_{Z}}=(u_1,u_2)$ and $V_{\a_{Z}}=(v_1,v_2)$. 
\end{defn}

\begin{defn}[$\pm 1$ distribution]
    We define $\o_{\pm1}$, the \emph{$\pm1$ distribution} to be that $x=1$ with probability $1/2$ and $-1$ otherwise if $x\sim\o_{\pm1}$.
\end{defn}

\begin{rmk}  
    The graph matrix $M_{\a,\o_{\pm1}}$ coincide with the definition of graph matrix $M_{\a}$ in the paper \cite{CP20}.
\end{rmk}

\begin{rmk}
    We will assume distribution $\o$ have mean $0$ and variance $1$ for the rest of the discussion.
\end{rmk}

\begin{thm}\label{thm:zshape+diagonal}
    Let $R$ be a random orthogonal matrix. Let $D, D'$ be random diagonal matrices where the diagonal entries $d_i,d_i'$ of $D,D'$ are independently drawn from distributions $\Omega$ and $\Omega'$, respectively. Let $\Omega$ be the singular value spectrum of $M_{\a_Z,\o_{\pm1}}$. Then $\dfrac{1}{n}\cdot DRD'$ has the same limiting distribution of singular values as the graph matrix $\dfrac{1}{n}\cdot M_{\a_Z,\o'}$.
\end{thm}

\begin{defn}[Definition 3.8 of \cite{AMP20}: Constraint graphs on $H(\alpha,2q)$]
	We define \\$\mathcal{C}_{(\alpha,\oa,2q)} = \left\{C(\phi): \phi: V(\alpha,2q) \to [n] \text{ is piecewise injective}\right\}$ to be the set of all possible constraint graphs on $V(\alpha,2q)$ which come from a piecewise injective map $\phi: V(\alpha,2q) \to [n]$.
		
	Given a constraint graph $C \in \mathcal{C}_{(\alpha,\oa,2q)}$, we make the following definitions:
	\begin{enumerate}
		\item We define $N(C) = \abs{\left\{\phi: V(\alpha,2q) \to [n]: \phi \text{ is piecewise injective}, C(\phi) = C\right\}}$.
		\item We define $\val(C) = \Ebb\[\chi_{\phi\(E(\alpha,2q)\)}(G)\]$ where $\phi: V(\alpha,2q) \to [n]$ is any piecewise injective map such that $C(\phi)=C$.
	\end{enumerate}
		
	We say that a constraint graph $C$ on $H(\a,2q)$ is \textit{nonzero-valued} if $\val(C)\neq 0$.
\end{defn}

\begin{defn}[Dominant Constraint Graphs]\label{defn:dominant constraint graph}
    We say a constraint graph $C \in \C_{\a,\oa,2q}$ is a \textit{dominant constraint graph} if $\val(C) \neq 0$ and $
\abs{E(C)}=\min\left\{\abs{E(C')}: C' \in \C_{\a,\oa,2q}, \val(C') \neq 0\right\}$. We denote the set of dominant constraint graphs in $\C_{\a,\oa,2q}$ to be $\D_{\a,\oa,2q}$.
\end{defn}

\begin{defn}\label{defn:weighted sum of dominant constraint grpah}
    We define the \emph{weighted sum of the dominant constraint graphs $C\in\C_{\a,\oa,2q}$} to be 
    \begin{equation*}
        %W\(\D_{\a,\oa,2q}\) = \sum_{\substack{C\in\C_{\a,\oa,2q}:\\ C\text{ dominant}}} \val(C).
        W\(\D_{\a,\oa,2q}\) = \sum_{C\in\D_{\a,\oa,2q}} \val(C).
    \end{equation*}
\end{defn}

\begin{rmk}
    When $\oa=\o_{\pm1}$, $W\(\D_{\a,\oa,2q}\)=
    \abs{\D_{\a,\oa,2q}} =$ the number of dominant constraint graphs in $\C_{\a,\oa,2q}$.
\end{rmk}
